WhiteFox: White-Box Compiler Fuzzing Empowered by Large Language Models

Compiler correctness is crucial, as miscompilation can falsify program behaviors, leading to serious consequences. Fuzzing has been studied to uncover compiler defects. However, compiler fuzzing remains challenging: Existing arts focus on black- and grey-box fuzzing, which generates tests without sufficient understanding of internal compiler behaviors. Meanwhile, traditional white-box techniques, like symbolic execution, are computationally inapplicable to the giant codebase of compilers. Recent advances demonstrate that Large Language Models (LLMs) excel in code generation/understanding tasks. Nonetheless, guiding LLMs with compiler source-code information remains a missing piece of research in compiler testing. To this end, we propose WhiteFox, the first white-box compiler fuzzer using LLMs with source-code information to test compiler optimization, with a spotlight on detecting deep logic bugs in the deep learning (DL) compilers. WhiteFox adopts a multi-agent framework: an LLM-based analysis agent examines the low-level optimization source code and produces requirements on the high-level test programs that can trigger the optimization; an LLM-based generation agent produces test programs based on the summarized requirements. Additionally, optimization-triggering tests are used as feedback to enhance the generation on the fly. Our evaluation on the three most popular DL compilers (i.e., PyTorch Inductor, TensorFlow-XLA, and TensorFlow Lite) shows WhiteFox can generate high-quality test programs to exercise deep optimizations, practicing up to 8X more than state-of-the-art fuzzers. WhiteFox has found 101 bugs for the DL compilers, with 92 confirmed as previously unknown and 70 fixed. WhiteFox has been acknowledged by the PyTorch team and is being incorporated into its development workflow. Beyond DL compilers, WhiteFox can also be adapted for compilers in different domains.

==> motivation.tex <==

\begin{figure*}[t]
    \centering
\includegraphics[keepaspectratio=true,width=0.9\textwidth]{figures/motivation.pdf}
    \caption{Motivating example.}
    \label{fig:motivation}
\end{figure*}

\reyhan{This section requires an illustrative example to introduce the terms, to which you can refer when explaining the approach. Without it, the approach section is hard to read.}


To illustrate \tech{}, we present a motivating example in this section, which shown in Figure~\ref{fig:motivation}.
The left side of the figure shows the implementation source code of the optimization \CodeIn{permute\_linear\_fusion} in \ptinductor, which fuses the \CodeIn{permute} and \CodeIn{linear} operators when \textit{``the permute method is invoked on an input tensor with more than 2 dimensions, and it swaps the last two dimensions of this tensor''}.
Such constraints are written in the implementation code explicitly.
When applying fuzzing techniques to test this optimization, black/grey-box fuzzing faces challenges: 1) generating valid models, and 2) ensuring the models with \CodeIn{permute} and \CodeIn{linear} operators align with the constraints.
The difficulties arise because these fuzzing approaches generate input models without using source code information as guidance.
Specifically, both black-box and grey-box fuzzing are unaware that the models should include the \CodeIn{permute} and \CodeIn{linear} operators.
Furthermore, the \CodeIn{permute} method is designed to swap the last two dimensions of a tensor.
As a result, the generated models often fail validation checks and are \textit{unable} to trigger the target optimization.
While traditional white-box fuzzing can explore new paths by solving constraints extracted from the source code, it requires modeling all internal behaviors, such as data structures.
This is often impractical in the context of modern compilers.
Back to the \CodeIn{permute\_linear\_fusion} optimization, it involves numerous complex data structures like \CodeIn{torch.fx.GraphModule} and \CodeIn{torch.fx.Node}.
These structures are further composed of several other intricate classes.
Given this complexity, it is not practical to model the behaviors of each component.
Plus, in the \CodeIn{check\_permute} function, \chenyuan{is such permutation check easy to be collected and solved in white-box fuzzing?}

Can we scale the white-fox fuzzing to fully test optimizations in modern compilers?
We address this question based on the insight that \llm{s} excel in both code comprehension and generation.
They have also been demonstrated to effectively fuzz a variety of software systems.
Thus, for the \CodeIn{permute\_linear\_fusion}, different from traditional white-box fuzzing, \tech leverages \llm{s} to infer the requirements for the models that could trigger it based on the source code information, as highlighted in the yellow text box of Figure~\ref{fig:motivation}.
Then, \tech utilizes the generated requirement description to further guide \llm{s} to generate the corresponding inputs, which are \pt models in this case.
In our experiments, the generated tests indeed triggered the \CodeIn{permute\_linear\_fusion} optimization and even detected a \textit{high-priority} bug in it!

==> pre.tex <==

\chenyuan{\textbf{NOTE: This section will be deleted}}

Most compilers perform optimization on the compiler-dependent internal representation (\ir).
Even in the optimizations in the same system, the \ir{s} could be different.
For instance, \chenyuan{todo}
Besides, the input to the system is not in the format of \ir.

In general, there exist two kinds of approaches for searching for a matching pattern within the input.

\textbf{Pattern Mapping} is to verify whether the input contains a specific pattern pre-defined in the source code.
If so, the optimizer would perform some modifications, such as replacing the pattern with an operator with better performance.
Mostly, the pattern to be matched is in the format of a self-defined data structure.
For example, the optimizer \inductor in \pt writes the pattern with \CodeIn{CallFunction} class shown in Figure~\ref{fig:map-example}, which has a method \CodeIn{\_match} to check whether the input has such a pattern.\lingming{there is no `match' in the code snippet, which is a bit confusing}\chenyuan{added}

\begin{figure}[h]
    \centering
    \includegraphics[keepaspectratio=true,width=0.5\columnwidth]{figures/mapping-example.pdf}
    \caption{Example of pattern mapping.}
    \label{fig:map-example}
\end{figure}



\textbf{Pattern Checking} is to check the requirements of the pattern step-by-step, which provides a greater degree of flexibility.
Figure~\ref{fig:check-example} presents the source code of \CodeIn{permute\_linear\_fusion} function in \inductor, which checks whether the \CodeIn{input\_node} is a \CodeIn{permute} operation only swapping the last two dimensions and leaving others unchanged.
Compared to pattern mapping, the checking function is able to match more complicated patterns, such as the permutation swapping the last two dimensions, which is pretty hard to be mapped with \CodeIn{CallFunction} structure.

\lingming{what's the diff between pattern mapping and checking? can they overlap with each other?}
\chenyuan{I think mapping could be considered as a special checking that directly checks whether a specific pattern in the model. However, the mapping is more structural, and it will reuse the same \CodeIn{\_match} method as the ``if conditions'' of checking. Many pattern mappings share the same code. That said, if we could unfold all the code of \CodeIn{CallFunction} to make the code for each mapping unique, they can be considered as checking}\yinlin{I think pattern matching is a simple type of pattern checking, because it can only handle ``lexical'' matching? If written in a function like ``check\_permute'', it allows for more complicated checking, such as control flows, more convoluted constraints like ``input().rank-2'', and even filters written as another helper function. }
\chenyuan{I agree, matching has less flexibility and expressiveness than checking}

\chenyuan{@lingming, do you think we need to distinguish them? The issue if we don't distinguish them is that it is hard to claim we design different one-shot example for them}


\begin{figure}[h]
    \centering
    \includegraphics[keepaspectratio=true,width=0.5\columnwidth]{figures/check-example.pdf}
    \caption{Example of pattern checking.}
    \label{fig:check-example}
\end{figure}

